Underactuated Two Stage CubeSat Control Law

This paper details the implementation of a two stage underactuated control law for a CubeSat to reduce all angular rates to zero. This CubeSat has a diagonal inertia matrix where the principal axes of inertia are not equal. This is needed for momentum transfer between axes as shown by previous work in this area. The momentum transfer will provide control to the uncontrolled axis to reduce all angular rates of a CubeSat to zero. The underactuated control utilizes actuators on only two axes but still reduces all three angular rates to zero. The first stage utilizes one axis to control the uncontrolled axis to zero and then the second stage reduces the other two axes to zero. This control law is similar to other piece wise control laws but the difference lies in only using one axis to control the third axis. The control mechanism is an integrated two axis propulsion system. The control law is derived to show its viability and a fully non-linear six degree of freedom simulation tool is utilized to verify the derivation. The simulation tool is developed by the Facility of Aerospace Systems and Technology. Simulation results are shown for a 1U, 2U, and 6U CubeSat with three and two axis control. The two stage underactuated control law is compared to a proportional controller as well as a feedback linearization control law for comparison.

==> Sections/Simulation_OLD.tex <==
%P Control and FL works for 1U,2U upright/side,6U if rank=3
%P Control and FL 1U,2U upright/side,6U if rank=2
%2-stage 1U,2U upright/side,6U if rank=2
%Make table for all control laws

%With the multiple control laws explained in detail, 
Simulation results of the 1U, 2U, and 6U CubeSat using the control laws from the previous section are presented below. The simulation software used to simulate the CubeSat is the Facility for Aerospace Systems and Technologies Configurable Autopilot and Simulation Software Tool (FASTCASST). The FASTCASST software is an open-source software suite written in the C++ programming language and has multiple modes to allow for extensive testing of both software and hardware. The full software suite is stored on GitHub as a repository \cite{FASTCASST_Repo}. The modes of the FASTCASST software include simulation only (SIMONLY) mode, software-in-the-loop (SIL) simulation mode, hardware-in-the-loop (HIL) mode, and an autopilot mode (AUTO) for real hardware. However, the SIMONLY mode was the only mode used to simulate this CubeSat. The SIMONLY mode simulates a vehicle over a specific period of time. The simulation simulates the vehicle dynamics and control system within a virtual environment. The translational dynamics are integrated using point mass physics and a point mass model for the gravitational field of the Earth. The rotational dynamics were explained in a previous section. The dynamics and state of the simulated vehicle are recorded and saved upon completion of the simulation. Further explanation of the software architecture and simulation dynamics can be seen in the previous works \cite{FASTKit_Aviation,MJ_Thesis}.

The simulation uses quaternions in a standard six degree of freedom rigid body model. The initial conditions of the CubeSat are saved in a text file and are read into the FASTCASST software at the start of the simulation. The initial conditions of the CubeSat are shown in the table below. The CubeSat is simulated in a low Earth orbit (LEO) of 500 kilometers. The orbit is a circular orbit about the equator of the Earth. It should be noted that the simulation is only run for 10 seconds when using the proportional and feedback linearized control laws and for 20 seconds when using the two-stage control law. The simulation time does not show the full orbit in order to show the angular velocities converging to zero when the CubeSat detumbles upon ejection from the launch vehicle.

\begin{table}[H]
 \centering
 \caption{Initial Conditions of the CubeSat}
\begin{tabular}{ |c|c|  }
 \hline
 \multicolumn{2}{|c|}{\textbf{Initial Conditions for Six DOF Model with Quaternions}} \\
 \hline
 6871393.0 & Initial X Position (m) \\
 \hline
 0.0 & Initial Y Position (m) \\
 \hline
 0.0 & Initial Z Position (m) \\
 \hline
 1.0 & Quaternion 0 \\
 \hline
 0.0 & Quaternion 1 \\
 \hline
 0.0 & Quaternion 2 \\
 \hline
 0.0 & Quaternion 3 \\
 \hline
 0.0 & Initial Xbody Velocity (m/s) \\
 \hline
 7616.18 & Initial Ybody Velocity (m/s) \\
 \hline
 0.0 & Initial Zbody Velocity (m/s) \\
 \hline
 0.2 & Initial Roll Rate (rad/s) \\
 \hline
 0.2 & Initial Pitch Rate (rad/s) \\
 \hline
 0.2 & Initial Yaw Rate (rad/s) \\
 \hline
\end{tabular}
\label{t:IC_CubeSat}
\end{table}

\noindent The inertial refernce frame of the CubeSat is Earth-Centered Inertial (ECI) with the x-axis points towards the point on the surface of the Earth where the prime meridian and equator intersect. This is why there is an initial x position instead of a z position. The initial x position also does accounts for the radius of the Earth, 6371393 meters. This means the CubeSat is initially 500 km above the surface of the Earth. The z-axis of the ECI frame points out of the North pole and the y-axis completes the triad. The initial angular velocities were chosen from the a standard deployment rate of 10 degrees per second upon ejection from the launch vehicle. The only conditions that change between the different size CubeSats are the mass moments of inertia and the total mass. The mass moments of inertia and the total mass of each CubeSat is shown in the table below. Note the y component of velocity is calculated from the orbit of the CubeSat to be placed in a perfectly circular orbit around the equator.

\begin{table}[H]
 \centering
 \caption{CubeSat Mass Moment of Inertia and Total Mass}
\begin{tabular}{ |c|c|c|c|c|  }
 \hline
 \textbf{CubeSat Size} & Mass (kg) & \textbf{$I_{x} (kg \cdot m^{2})$} & \textbf{$I_{y} (kg \cdot m^{2})$} & \textbf{$I_{z} (kg \cdot m^{2})$} \\
 \hline
 \textbf{1U} & 2 & 0.0033 & 0.0033 & 0.0033 \\
 \hline
 \textbf{2U, Upright} & 4 & 0.0167 & 0.0167 & 0.0067 \\
 \hline
 \textbf{2U, Sideways} & 4 & 0.0067 & 0.0167 & 0.0167 \\
 \hline
 \textbf{6U} & 12 & 0.13 & 0.10 & 0.05 \\
 \hline
\end{tabular}
\label{t:Masses_Intertias}
\end{table}

The actuators used on the underactuated CubeSat will be modeled after a thruster which will provide three-axis control. However, the thruster will be limited to two-axis control hen specified. The CubeSat thruster modeled is the VACCO Integrated Propulsion System (IPS) \cite{gimballed_thruster}. The IPS is a complete propulsion module with a plug-and-play capability. The IPS has four individual thrusters that are pointed inward 7 degrees off center. With each thruster pointed off center, three-axis control is possible but is not used when the satellite is underactuated. Each thruster provides 1 newton of thrust for a total axial thrust of 4 newtons and a total impulse of 12,000 newton-seconds \cite{gimballed_thruster}. An image of the thruster is shown below.

\begin{figure}[H]
\centering
\includegraphics[width=0.6\textwidth]{Figures/Integrated-Propulsion-System.jpg}
\caption{VACCO Integrated Propulsion System\cite{gimballed_thruster}}
\label{fig:VaccoThruster}
\end{figure}

Table \ref{t:ControlScheme} shown below gives a quick summary of which control laws succeeded in driving all angular rates to zero for the different CubeSat configurations. For the fully actuated CubeSat where the rank of the moment vector $\vec{M}$ is equal to three ($r(\vec{M})=3$), the proportional and feedback linearized control laws were successful in driving all angular rates to zero. For the fully actuated scenario the Two-Stage control law was not simulation. For the scenario where the rank of the moment vector $\vec{M}$ is equal to two ($r(\vec{M})=2$), the Two stage control law was effective in driving all angular rates to zero provided the roll and pitch axes of inertia were not identical. 

Boxes marked with green check marks show that the control law was successful for the CubeSat configuration, boxes marked red Xs show that the control law did not work for the CubeSat configuration, and unmarked boxes with dashes show the control law was not simulated for the CubeSat configuration. 

%were simulated. When the CubeSat was underactuated, the proportional, feedback linearized, and two-stage control laws were used. The two-stage control law was design for an underactuated CubeSat which is why it was not simulated for a fully actuated CubeSat. The results shown in the table are shown and discussed in the following Subsections.

\begin{table}[H]
 \centering
 \caption{Control Law and CubeSat Configurations}
\begin{tabular}{ |c|c|c|c|  }
 \hline
 \multicolumn{4}{|c|}{\textbf{Fully Actuated, $r(\vec{M})=3$}} \\
 \hline
 \textbf{CubeSat Size} & \textbf{Proportional Control} & \textbf{Feedback Linearized Control} & \textbf{Two-Stage Control} \\
 \hline
 \textbf{1U} & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & - \\
 \hline
 \textbf{2U, Upright} & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & - \\
 \hline
 \textbf{2U, Sideways} & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & - \\
 \hline
 \textbf{6U} & \cellcolor{green} \checkmark & \cellcolor{green} \checkmark & - \\
 \hline
 \multicolumn{4}{|c|}{\textbf{Underactuated Actuated, $r(\vec{M})=2$}} \\
 \hline
 \textbf{CubeSat Size} & \textbf{Proportional Control} & \textbf{Feedback Linearized Control} & \textbf{Two-Stage Control} \\
 \hline
 \textbf{1U} & \cellcolor{red} X & \cellcolor{red} X & \cellcolor{red} X \\
 \hline
 \textbf{2U, Upright} & \cellcolor{red} X &  \cellcolor{red} X & \cellcolor{red} X \\
 \hline
 \textbf{2U, Sideways} & \cellcolor{red} X &  \cellcolor{red} X & \cellcolor{green} \checkmark \\
 \hline
 \textbf{6U} & \cellcolor{red} X &  \cellcolor{red} X & \cellcolor{green} \checkmark \\
 \hline
\end{tabular}
\label{t:ControlScheme}
\end{table}

\subsection{Fully Actuated CubeSat Simulation Results}
Before simulating an underactuated CubeSat, the proportional, feedback linearized, and two-stage controllers were simulated on a 1U, 2U, and 6U CubeSat that are fully actuated. Simulating a fully actuated CubeSat ensures the controllers are working properly. The results for a 1U CubeSat are shown below. Fig. \ref{fig:1U_PropFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 radians per second (rad/s). As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. Fig. \ref{fig:1U_PropFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/36_PDFsam_1U_P_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:1U_PropFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/37_PDFsam_1U_P_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:1U_PropFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a 1U CubeSat Using the Proportional Control Law}
        \label{fig:1U_PropFully}
\end{figure}

The results of the proportional controller for a 2U Upright CubeSat are shown below. Fig. \ref{fig:2U_Upright_PropFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. Fig. \ref{fig:2U_Upright_PropFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. It should be noted that the z moment is smaller than the x and y moments due to the smaller mass moment of inertia about the z axis. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/36_PDFsam_2U_Upright_P_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Upright_PropFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/37_PDFsam_2U_Upright_P_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Upright_PropFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Upright 2U CubeSat Using the Proportional Control Law}
        \label{fig:2U_Upright_PropFully}
\end{figure}

The results of the proportional controller for a 2U Sideways CubeSat are shown below. Fig. \ref{fig:2U_Sideways_PropFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. Fig. \ref{fig:2U_Sideways_PropFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. It should be noted that the x moment is smaller than the y and z moments due to the smaller mass moment of inertia about the x axis. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/36_PDFsam_2U_Sideways_P_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Sideways_PropFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/37_PDFsam_2U_Sideways_P_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Sideways_PropFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a Sideways 2U CubeSat Using the Proportional Control Law}
        \label{fig:2U_Sideways_PropFully}
\end{figure}

The results of the proportional controller for a 6U CubeSat are shown below. Fig. \ref{fig:6U_PropFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. It should be noted that the x component takes longer than the y component and y component takes longer than the z component due to the mass moments of inertia of the CubeSat. Fig. \ref{fig:6U_PropFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. It should be noted that the x moment takes longer than the y moment and y moment takes longer than the z moment due to the mass moments of inertia of the CubeSat. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/36_PDFsam_6U_P_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:6U_PropFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Fully/37_PDFsam_6U_P_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:6U_PropFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a 6U CubeSat Using the Proportional Control Law}
        \label{fig:6U_PropFully}
\end{figure}

The feedback linearized controller was simulated after the proportional controller. The results of the feedback linearized controller for a 1U CubeSat are shown below. Fig. \ref{fig:1U_FLFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. Fig. \ref{fig:1U_FLFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/36_PDFsam_1U_FL_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:1U_FLFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/37_PDFsam_1U_FL_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:1U_FLFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a 1U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:1U_FLFully}
\end{figure}

The results of the feedback linearized controller for a 2U Upright CubeSat are shown below. Fig. \ref{fig:2U_Upright_FLFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. Fig. \ref{fig:2U_Upright_FLFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. It should be noted that the z moment is smaller than the x
and y moments due to the smaller mass moment of inertia about the z axis. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/36_PDFsam_2U_Upright_FL_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Upright_FLFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/37_PDFsam_2U_Upright_FL_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Upright_FLFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Upright 2U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:2U_Upright_FLFully}
\end{figure}

The results of the feedback linearized controller for a 2U Sideways CubeSat are shown below. Fig. \ref{fig:2U_Sideways_FLFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. Fig. \ref{fig:2U_Sideways_FLFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. It should be noted that the x moment is smaller than the y and z moments due to the smaller mass moment of inertia about the x axis. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/36_PDFsam_2U_Sideways_FL_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Sideways_FLFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/37_PDFsam_2U_Sideways_FL_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Sideways_FLFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a Sideways 2U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:2U_Sideways_FLFully}
\end{figure}

The results of the feedback linearized controller for a 6U CubeSat are shown below. Fig. \ref{fig:6U_FLFully_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, each component of the angular velocity vector is driven to zero showing that the proportional control law works for this CubeSat configuration. It should be noted that the x component takes longer than the y component and y component takes longer than the z component due to the mass moments of inertia of the CubeSat Fig. \ref{fig:6U_FLFully_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is fully actuated, the control moments about the x, y, and z axes are shown. Each control moment has an initial spike as the angular velocity vector is driven to zero. It should be noted that the x moment takes longer than the y moment and y moment takes longer than the z moment due to the mass moments of inertia of the CubeSat. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/36_PDFsam_6U_FL_Fully.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:6U_FLFully_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Fully/37_PDFsam_6U_FL_Fully.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:6U_FLFully_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a 6U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:6U_FLFully}
\end{figure}

\subsection{Underactuated Actuated CubeSat Simulation Results}
With all controllers shown to have worked on a fully actuated CubeSat, the controllers were then tested on a 1U, 2U, and 6U CubeSat that are underactuated. The proportional controller was simulated first, and the results for a 1U CubeSat are shown below. Fig. \ref{fig:1U_PropUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:1U_PropUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/35_PDFsam_1U_P_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:1U_PropUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/36_PDFsam_1U_P_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:1U_PropUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated 1U CubeSat Using the Proportional Control Law}
        \label{fig:1U_PropUnder}
\end{figure}

The results of the proportional controller for a 2U Upright CubeSat are shown below. Fig. \ref{fig:2U_Upright_PropUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:2U_Upright_PropUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/35_PDFsam_2U_Upright_P_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Upright_PropUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/36_PDFsam_2U_Upright_P_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Upright_PropUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated Upright 2U CubeSat Using the Proportional Control Law}
        \label{fig:2U_Upright_PropUnder}
\end{figure}

The results of the proportional controller for a 2U Sideways CubeSat are shown below. Fig. \ref{fig:2U_Sideways_PropUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:2U_Sideways_PropUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/35_PDFsam_2U_Sideways_P_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Sideways_PropUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/36_PDFsam_2U_Sideways_P_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Sideways_PropUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated Sideways 2U CubeSat Using the Proportional Control Law}
        \label{fig:2U_Sideways_PropUnder}
\end{figure}

The results of the proportional controller for a 6U CubeSat are shown below. Fig. \ref{fig:6U_PropUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. It should be noted that the x component takes longer to converge to zero due to the mass moments of inertia of the CubeSat. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:6U_PropUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/35_PDFsam_6U_P_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:6U_PropUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Proportional_Under/36_PDFsam_6U_P_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:6U_PropUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated 6U CubeSat Using the Proportional Control Law}
        \label{fig:6U_PropUnder}
\end{figure}

The feedback linearized controller was simulated after the proportional controller. The results of the feedback linearized controller for a 1U CubeSat are shown below. Fig. \ref{fig:1U_FLUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:1U_FLUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/35_PDFsam_1U_FL_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:1U_FLUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/36_PDFsam_1U_FL_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:1U_FLUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated 1U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:1U_FLUnder}
\end{figure}

The results of the feedback linearized controller for a 2U Upright CubeSat are shown below. Fig. \ref{fig:2U_Upright_FLUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:2U_Upright_FLUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/35_PDFsam_2U_Upright_FL_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Upright_FLUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/36_PDFsam_2U_Upright_FL_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Upright_FLUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated Upright 2U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:2U_Upright_FLUnder}
\end{figure}

The results of the feedback linearized controller for a 2U Sideways CubeSat are shown below. Fig. \ref{fig:2U_Sideways_FLUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:2U_Sideways_FLUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/35_PDFsam_2U_Sideways_FL_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Sideways_FLUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/36_PDFsam_2U_Sideways_FL_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:2U_Sideways_FLUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated Sideways 2U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:2U_Sideways_FLUnder}
\end{figure}

The results of the feedback linearized controller for a 6U CubeSat are shown below. Fig. \ref{fig:6U_FLUnder_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. As the simulation runs, the x and y components of the angular velocity vector are driven to zero. Since the CubeSat is underactuated, the z component does not given driven to zero and stays at 0.2 rad/s due to there being no control moment about the z-axis. It should be noted that the x component takes longer to converge to zero due to the mass moments of inertia of the CubeSat. Since the angular velocity vector does not get driven to zero, the proportional control law does not work for this underactuated CubeSat configuration. Fig. \ref{fig:6U_FLUnder_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, the control moments about the x and y axes are shown. Each control moment has an initial spike as the x and y components of the angular velocity vector are driven to zero. The control moments converge to zero when the angular velocity vector is zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/35_PDFsam_6U_FL_Under.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:6U_FLUnder_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/Feedback_Under/36_PDFsam_6U_FL_Under.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:6U_FLUnder_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Underactuated 6U CubeSat Using the Feedback Linearized Control Law}
        \label{fig:6U_FLUnder}
\end{figure}

Since neither the proportional nor the feedback linearized controllers were shown to have worked with an underactuated CubeSat, the two-stage control scheme was simulated next. The results of the two-stage control scheme for a 1U CubeSat are shown below. Fig. \ref{fig:1U_TwoStage_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 radians per second (rad/s). As the simulation runs and the first stage begins, the x component of the angular velocity vector increases to the commanded value of 0.5 rad/s. The z component stays at 0.2 rad/s, and the y component decreases to -1 rad/s. Since the mass moments of inertia are the same for the 1U CubeSat, the y and z components are never driven to zero, and the second stage of the control law never begins. Since the control law never enters the second stage and the angular velocity vector is never driven to zero, the two-stage control scheme will not work. Momentum transfer does occur in the x and y components of the angular velocity vector, but neither component is driven to zero. Fig. \ref{fig:1U_TwoStage_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, only the x and y moments are shown. There is an initial spike in both the x and y moments as the controller tries to drive the angular velocity vector of the CubeSat to zero. The control moments converge to zero when the components of the angular velocity vector level out after momemtum transfer has occured.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/35_PDFsam_1U_TwoStage.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:1U_TwoStage_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/36_PDFsam_1U_TwoStage.pdf}
         \caption{\centering Control Moment Components}
         \label{fig:1U_TwoStage_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a 1U CubeSat Using the Two-Stage Control Law}
        \label{fig:1U_TwoStage}
\end{figure}

The results of the two-stage controller for a 2U Upright CubeSat are shown below. Fig. \ref{fig:2U_Upright_TwoStage_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. Similar to the 1U CubeSat when the first stage begins, the x component of the angular velocity vector increases to the commanded value of 0.5 rad/s, the z component stays at 0.2 rad/s, and the y component decreases to -1 rad/s. This is due to the mass moments of inertia along the x and y axes being the same, so the second stage of the control law never begins. The two-stage control scheme will not work for this CubeSat configuration. Momentum transfer does occur in the x and y components of the angular velocity vector, but neither component is driven to zero. Fig. \ref{fig:2U_Upright_TwoStage_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, only the x and y moments are shown. Similar to the 1U CubeSat, there is an initial spike in both the x and y moments as the controller tries to drive the angular velocity vector of the CubeSat to zero. The control moments converge to zero when the components of the angular velocity vector level out after momemtum transfer has occured.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/35_PDFsam_2U_Upright_TwoStage.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Upright_TwoStage_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/36_PDFsam_2U_Upright_TwoStage.pdf}
         \caption{\centering Total Moment Components}
         \label{fig:2U_Upright_TwoStage_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of an Upright 2U CubeSat Using the Two-Stage Control Law}
        \label{fig:2U_Upright_TwoStage}
\end{figure}

The results of the two-stage controller for a 2U Sideways CubeSat are shown below. Fig. \ref{fig:2U_Sideways_TwoStage_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. At the start of the first stage, the x component of the angular velocity vector increases to the commanded value of 0.5 rad/s. The x component holds steady at this value while the z component transfers its momentum to the y component as seen with the rapid increase of the y component at the start of the simulation. As the momentum transfer occurs, the y component is also driven to a value of zero along with the z component. Once the z component converges to zero shortly before 5 seconds, the second stage begins, and the x component is driven to zero. Since the mass moments of inertia along the x and y axes are different, all components of the angular velocity vector are driven to zero, and the two-stage control scheme is shown to work for this CubeSat configuration. Fig. \ref{fig:2U_Sideways_TwoStage_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, only the x and y moments are shown. The x moment is shown to have an initial spike as the x component of the angular velocity vector is driven to 0.5 rad/s. The y moment is also shown to have an initial spike as the y component of the angular velocity vector grows with the momentum transfer. As the y component drives to zero, it overshoots and becomes negative. At this point the y moment also becomes negative to bring the y component back to zero. At shortly before 5 seconds, the x moment spikes again as the second stage starts and the x component of the angular velocity vector is driven to zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/35_PDFsam_2U_Sideways_TwoStage.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:2U_Sideways_TwoStage_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/36_PDFsam_2U_Sideways_TwoStage.pdf}
         \caption{\centering Total Moment Components}
         \label{fig:2U_Sideways_TwoStage_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a Sideways 2U CubeSat Using the Two-Stage Control Law}
        \label{fig:2U_Sideways_TwoStage}
\end{figure}

The results of the two-stage controller for a 6U CubeSat are shown below. Fig. \ref{fig:6U_TwoStage_PQR} shows the components of the angular velocity vector of the CubeSat. All of the components start at the initial condition of 0.2 rad/s. At the start of the first stage, the x component of the angular velocity vector increases to the commanded value of 0.5 rad/s similar to the Sideways 2U CubeSat. The x component holds steady at this value while the z component transfers its momentum to the y component as seen with the rapid decrease of the y component at the start of the simulation. As the momentum transfer occurs, the y component is also driven to a value of zero along with the z component. Once the z component converges to zero at 16 seconds, the second stage begins, and the x component is driven to zero. Since the mass moments of inertia for the 6U CubeSat are much larger than the sideways 2U CubeSat, the y and z components of the angular velocity vector take longer to converge to zero and oscillate around zero until they converge. All components of the angular velocity vector are driven to zero, and the two-stage control scheme is shown to work for this CubeSat configuration. Fig. \ref{fig:6U_TwoStage_LMN} shows the control moments of the CubeSat from the thruster. Since the CubeSat is underactuated, only the x and y moments are shown. The x moment is shown to have an initial spike as the x component of the angular velocity vector is driven to 0.5 rad/s. The y moment is also shown to have an initial spike as the y component of the angular velocity vector decreases below zero with the momentum transfer. As the y component drives to zero, it overshoots and oscillates around zero. At this point the y moment also oscillates to bring the y component back to zero. At 16 seconds, the x moment spikes again as the second stage starts and the x component of the angular velocity vector is driven to zero.

\begin{figure}[H]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/35_PDFsam_6U_TwoStage.pdf}
         \caption{\centering Angular Velocity Components}
         \label{fig:6U_TwoStage_PQR}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Figures/TwoStage/36_PDFsam_6U_TwoStage.pdf}
         \caption{\centering Total Moment Components}
         \label{fig:6U_TwoStage_LMN}
     \end{subfigure}
        \caption{Angular Velocity and Total Moment Vectors of a 6U CubeSat Using the Two-Stage Control Law}
        \label{fig:6U_TwoStage}
\end{figure}
